Deep Optimal Sensor Placement for Black Box Stochastic Simulations

Selecting cost-effective optimal sensor configurations for subsequent inference of parameters in black-box stochastic systems faces significant computational barriers. We propose a novel and robust approach, modelling the joint distribution over input parameters and solution with a joint energy-based model, trained on simulation data. Unlike existing simulation-based inference approaches, which must be tied to a specific set of point evaluations, we learn a functional representation of parameters and solution. This is used as a resolution-independent plug-and-play surrogate for the joint distribution, which can be conditioned over any set of points, permitting an efficient approach to sensor placement. We demonstrate the validity of our framework on a variety of stochastic problems, showing that our method provides highly informative sensor locations at a lower computational cost compared to conventional approaches.

==> auxiliary_tex_files/application_BED.tex <==
\subsection{Bayesian Adaptive Design}
%One of the main motivations of our approach lies in Bayesian experimental design.
One of the main motivations for our approach lies in Bayesian experimental design, which can be carried out efficiently because we have a resolution-independent surrogate for the joint distribution $p_\theta(\mathbf{z}_\kappa, \mathbf{z}_u)$ capable of modelling stochastic associations.
% Specifically, we seek to determine optimal sparse sensor placement positions $\xib = \{\xib_1, \xib_2, \dots, \xib_D\}$ for the inference of $(\kappa, u= \mathcal G(\kappa))$ based on $\mathbf y = u(\xib)+\boldsymbol\eta$. 
The goal of BED is to determine optimal sparse sensor placement positions $\xib = \{\xib_1, \xib_2, \dots, \xib_D\}$ for the inference of $(\kappa, u= \mathcal G(\kappa))$ based on $\mathbf y = u(\xib)+\boldsymbol\eta$.
We measure the utility of a sensor placement position by calculating the expected information gain over the prior as measured by relative entropy, i.e. we use the utility function $U(\xib) := \mathbb E_{p(\mathbf y\vert\xib)}\KL{(p(\mathbf z_\kappa, \mathbf z_u \vert \mathbf y, {\xib})}\,\Vert\,{p_\theta(\mathbf z_\kappa, \mathbf z_u)})$, which can be evaluated at any design point $\xib$ thanks to the INR component.  
Using Bayes theorem, the utility can be rewritten as 
\begin{equation*}
        U(\xib)= \mathbb{E}_{p_\theta(\mathbf{z}_\kappa, \mathbf{z}_u)p( \mathbf{y}|\mathbf{z}_\kappa, \mathbf{z}_u,\xib)}\left[\log\frac{p(\mathbf{y}|\mathbf{z}_\kappa, \mathbf{z}_u, \xib)}{p(\mathbf{y}|\xib)} \right].
\end{equation*}
%\textbf{Thanks to the INR component the utility function can be evaluated at any design point.}
Since $p(\mathbf{y}|\xib)$ is unknown,
a naive Monte Carlo estimation provides a nested Monte Carlo estimator \citep{Rainforth2018OnNM}, which approximates the inner and outer integrals of the utility but suffers from a slow rate of convergence. Therefore, following on \citet{pmlr-v108-foster20a}, we use the prior contrastive estimation (PCE) bound given by
\begin{align}\label{eq:pce_bound}
    \Hat U_{\text{PCE}}(\xib)  = \mathbb{E}\left[\log \frac{p(\mathbf y|\mathbf z_{\kappa, 0}, \mathbf z_{u, 0}, \mathbf \xib)}{\frac{1}{L+1}\sum_{l=0}^L  p(\mathbf y|\mathbf z_{\kappa,l}, \mathbf z_{u,l},\xib)}\right]
    % &=  - \mathbb{E}\left[\log \left(1+\sum_{l=1}^L \frac{p(\mathbf y|\mathbf z_{a,l}, \mathbf z_{u,l},\xib)}{p(\mathbf y|\mathbf z_{a,0}, \mathbf z_{u,0},\xib)}\right)\right] + C,
\end{align}
where the expectation is computed over the distribution $p_\theta(\mathbf z_{\kappa,0}, \mathbf z_{u,0})p(\mathbf y|\mathbf z_{\kappa,0}, \mathbf z_{u,0},\xib)p_\theta(\mathbf z_{\kappa,1:L}, \mathbf z_{u,1:L})$.
This alternative estimator significantly speeds up training and is a valid lower bound of the utility which becomes tight as $L\to\infty$ \citep{pmlr-v108-foster20a}. Further details are given in Appendix \ref{sec:bed_appendix}.

Moreover, the selection of optimal designs can be conducted sequentially, which leads to 
Bayesian adaptive design (BAD) \citep{rainforth2023modern}. This framework extends BED to adaptive scenarios by sequentially incorporating information collected throughout the experiment to guide the designs for future experiments.
That is, the utility is updated with the new information obtained after performing the experiment corresponding to the optimal design of the previous iteration. 
In settings where multiple experiments can be run in parallel, each step of the optimisation can select a batch of optimal designs instead of just one.
%Thus, the utility is updated after selecting one new optimal design
%New optimal designs can be selected one by one or in batches.
Considering the sequence of designs and outcomes up to step  $t$ of the experiment, denoted by $\{\xib_1, \dots, \xib_{t-1}\}$ and $\{\mathbf{y}_1,\dots, \mathbf{y}_{t-1}\}$, respectively, we aim to maximise the utility given the history $h_{t-1} = \{(\xib_k, \mathbf{y}_k)\}_{k=1}^{t-1}$,
\begin{equation*}
    {U}({\xib_t}|h_{t-1})=\mathbb{E}\left[ \log\frac{p(\mathbf{y}|\mathbf{z}_\kappa,\mathbf{z}_u, \xib_t, h_{t-1})}{p(\mathbf{y}|\xib_t, h_{t-1})}\right]\,,
\end{equation*}
where $h_0 = \emptyset$ and the expectation is over  $p(\mathbf{z}_\kappa,\mathbf{z}_u|h_{t-1}) p (\mathbf{y}_t|\mathbf{z}_\kappa,\mathbf{z}_u, \xib_t, h_{t-1})$. This can also be interpreted as the conventional utility with an updated prior and likelihood. However, in most cases $\mathbf{y}_t$ is independent of $h_{t-1}$ given $(\mathbf{z}_\kappa, \mathbf{z}_u, \xib_t)$, thus only the prior needs to be updated.

%The utility is sequentially optimised using Bayesian optimisation. For details, see Appendix \ref{sec:bed_appendix}.\pce{TO DO: explain how sequential updates are done}
